Creation of non-classical states of light in a chiral waveguide

Creating non-classical states of light from simple quantum systems together with classical resources is a challenging problem. We show how chiral emitters under a coherent drive can generate non-classical photon states. For our analysis, we select a specific temporal mode in the transmitted light field, resulting in a coupled master equation for the relevant mode and the chiral emitters. We characterise the mode's state by its Wigner function and show that the emission from the system predominantly produces mixtures of few-photon-added coherent states. We argue that these non-classical states are experimentally accessible and show their application for quantum metrology.

==> Creation of Non-classical states of light in a chiral waveguide Arxiv/Supp_Mat.tex <==
\onecolumngrid
\appendix
\section{Short bin density matrix}
\label{app:MasterEquation}
The density matrix $\rho_v$ of the photons in mode $v$ can be found by explicitly calculating each matrix element as
\begin{equation}
    (\rho_v)_{m,n} = \Big\langle |n\rangle\langle m| \Big\rangle
    = \frac{1}{\sqrt{n!m!}}
    \big\langle :(b_v^\dagger)^n e^{-b_v^\dagger b_v} b_v^m : \big\rangle.
    \label{eq:DensityGeneral}
\end{equation}
Here, $:f(b_v^\dagger, b_v):$ denotes the normal ordering of $f(b_v^\dagger, b_v)$.
Since
\begin{equation}
    b_v = \frac{1}{\sqrt{\tau}} \int_{t_0}^{t_0+\tau} dt
    \big( \alpha + \sqrt{\kappa} \sigma_\mathrm{chain}^-(t)\big),
\end{equation}
the relation~\eqref{eq:DensityGeneral} for $\rho_v$ generally yields out-of-time-ordered correlation functions and thus determining $\rho_v$ is impractical in most situations.
However, for $\kappa \tau \ll 1$ we may approximate $b_v \approx \sqrt{\tau}\big(\alpha + \sqrt{\kappa} \sigma_\mathrm{chain}^-(t_0)\big)$, and thus calculate $\rho_v$ from the emitters' density matrix at time $t_0$.

Assuming $M$ chiral emitter we can expand the expectation value in~\eqref{eq:DensityGeneral} as
\begin{align}
    \notag
    :(b_v^\dagger)^n e^{-b_v^\dagger b_v} b_v^m :
    &\ = \sqrt{\tau}^{n+m}\sum_{k=0}^\infty \frac{(-\tau)^k}{k!}
    \big(\alpha^* + \sqrt{\kappa} \sigma_\mathrm{chain}^+\big)^{n+k}
    \big(\alpha   + \sqrt{\kappa} \sigma_\mathrm{chain}^-\big)^{m+k} \\
%
    \notag
    &\ = \sqrt{\tau}^{n+m}
    \sum_{\tilde{n}=0}^M (\alpha^*)^{n-\tilde{n}} (\sqrt{\kappa} \sigma_\mathrm{chain}^+)^{\tilde{n}}
    \sum_{\tilde{m}=0}^M  \alpha^{m-\tilde{m}} (\sqrt{\kappa} \sigma_\mathrm{chain}^-)^{\tilde{m}}\\
    &\ \qquad\times
    \sum_{k=0}^\infty
    \frac{(-\tau |\alpha|^2)^k}{k!} \binom{n+k}{\tilde{n}}\binom{m+k}{\tilde{m}}.
\end{align}
Due to the coherent drive it is expected that $\rho_v$ possesses large overlap with $|\sqrt{\tau}\alpha\rangle$.
Therefore, we extract a factor $e^{-\tau|\alpha|^2}$ from the $k$-summation by inserting $1 = e^{-\tau |\alpha|^2} e^{\tau|\alpha|^2}$, expanding the positive exponential and thereon collecting all terms of equal power in $(\tau|\alpha|^2)^k$, resulting in
\begin{align}
    \notag
    :(b_v^\dagger)^n e^{-b_v^\dagger b_v} b_v^m :
    &\ =
    (\sqrt{\tau}\alpha^*)^n (\sqrt{\tau}\alpha)^m e^{-\tau|\alpha|^2}
    \sum_{\tilde{n}=0}^M \frac{1}{\tilde{n}!} \left(\frac{\sqrt{\kappa} \sigma_\mathrm{chain}^+}{\alpha^*}\right)^{\tilde{n}}
    \sum_{\tilde{m}=0}^M \frac{1}{\tilde{m}!} \left(\frac{\sqrt{\kappa} \sigma_\mathrm{chain}^-}{\alpha}\right)^{\tilde{m}}\\
    \notag
    &\quad\qquad\times
    \sum_{k=0}^\infty
    \frac{(\tau |\alpha|^2)^k}{k!} \sum_{i=0}^k (-1)^i \binom{k}{i} (n+i)^{\ff{\tilde{n}}} (m+i)^{\ff{\tilde{m}}} \\
%
    \notag
    &\ = \sqrt{n!m!}
    \langle m|\sqrt{\tau}\alpha\rangle\langle\sqrt{\tau}\alpha| n\rangle
    \sum_{\tilde{n}=0}^M \frac{1}{\tilde{n}!} \left(\frac{\sqrt{\kappa} \sigma_\mathrm{chain}^+}{\alpha^*}\right)^{\tilde{n}}
    \sum_{\tilde{m}=0}^M \frac{1}{\tilde{m}!} \left(\frac{\sqrt{\kappa} \sigma_\mathrm{chain}^-}{\alpha}\right)^{\tilde{m}}\\
    &\quad\qquad\times
    \sum_{k=0}^\infty
    \frac{(- \tau |\alpha|^2)^k}{k!} \fd^k\Big|_{x=0} (n+x)^{\ff{\tilde{n}}} (m+x)^{\ff{\tilde{m}}}.
    \label{eq:DensityIntermediate}
\end{align}
Here, we introduced $x^{\ff{n}} = x(x-1)\dots(x-n+1)$ the falling factorial, and the forward difference operator $\fd$, defined as $\fd f(x) = f(x+1) - f(x)$.
For the simplification in the second step we used
\begin{equation}
    (-1)^k\fd^k f(x) = \sum_{i=0}^k (-1)^i \binom{k}{i} f(x+i).
\end{equation}
Next, we eliminate $n$ and $m$ from~\eqref{eq:DensityIntermediate} by using the number operator $n|n\rangle = b^\dagger b |n\rangle$ and find the density matrix
\begin{align}
    \notag
    &\rho_v = \sum_{\tilde{n}=0}^M \sum_{\tilde{m}=0}^M
    \frac{1}{\tilde{n}!} \frac{1}{\tilde{m}!}
    \left\langle
    \left(\frac{\sqrt{\kappa} \sigma_\mathrm{chain}^+}{\alpha^*}\right)^{\tilde{n}}
    \left(\frac{\sqrt{\kappa} \sigma_\mathrm{chain}^-}{\alpha  }\right)^{\tilde{m}}
    \right\rangle\\
    \notag
    &\quad\qquad\times
    \sum_{k=0}^{\infty} \frac{(- \tau |\alpha|^2)^k}{k!} \fd^k\Big|_{x=0}
    (b^\dagger b + x)^{\ff{\tilde{m}}} |\sqrt{\tau}\alpha\rangle\langle\sqrt{\tau}\alpha| (b^\dagger b + x)^{\ff{\tilde{n}}}.
    \label{eq:DensityPre}
\end{align}
It already is evident that $\rho_v$ is generated from the coherent state $|\sqrt{\tau}\alpha\rangle\langle\sqrt{\tau}\alpha|$ by application of an operator which is a function in $b^\dagger b$.
Next, we show that this operator only adds up to $M$ photons to $\rho_v$ and find $\rho_v$ in a Fock-state-basis.

The algebra of finite differences with falling factorials posses many similarities to the derivatives of monomials, e.g.~$\fd x^{\ff{n}} = n x^{\ff{n-1}}$, and one finds the generalised product rule $\fd fg = (\fd f)g + f(\fd g) + (\fd f)(\fd g)$.
Thus it is evident that~\eqref{eq:DensityPre} will only consist of falling factorials of the number operator, which directly translate into normal ordered powers $(b^\dagger b)^{\ff{n}} = :(b^\dagger b)^n:$.
Therefore, $\rho_v$ in~\eqref{eq:DensityPre} is invariant under the set of replacements
\begin{align}
    \fd\Big|_{x=0} \ &\mapsto\quad
    (\partial_x + \partial_y + \partial_x\partial_y)\Big|_{x=0=y} \\
%
    (b^\dagger b + x)^{\ff{\tilde{m}}} |\sqrt{\tau} \alpha\rangle \ &\mapsto\quad
    :(b^\dagger b + x)^{\tilde{m}}: |\sqrt{\tau} \alpha\rangle
    = (\sqrt{\tau}\alpha b^\dagger + x)^{\tilde{m}} |\sqrt{\tau} \alpha\rangle
    = \mathcal{D}(\sqrt{\tau}\alpha)
    (\sqrt{\tau}\alpha b^\dagger + \tau|\alpha|^2 + x)^{\tilde{m}} |0\rangle
    \label{eq:ReplaceLeft}\\
%
    \langle\sqrt{\tau} \alpha| (b^\dagger b + x)^{\ff{\tilde{n}}} \ &\mapsto\quad
    \langle\sqrt{\tau} \alpha| :(b^\dagger b + y)^{\tilde{n}}:\  
    = \langle\sqrt{\tau} \alpha| (\sqrt{\tau}\alpha^* b + y)^{\tilde{n}}
    = \langle0| (\sqrt{\tau}\alpha^* b + \tau|\alpha|^2 + y)^{\tilde{n}}
    \mathcal{D}^\dagger(\sqrt{\tau}\alpha).
    \label{eq:ReplaceRight}
\end{align}
We now perform the $k$-summation, which yields two translation operators $T_{x,y}(-\tau|\alpha|^2)$ for $x, y$ and the operator $\exp(-\tau|\alpha|^2 \partial_x\partial_y)$.
The translation operators cancel the $\tau|\alpha|^2$ terms in \eqref{eq:ReplaceLeft} and~\eqref{eq:ReplaceRight}. After rescaling $x$, $y$, we end up with the density matrix
\begin{align}
    \notag
    \mathcal{D}^\dagger(\sqrt{\tau}\alpha) \rho_v
    \mathcal{D}(\sqrt{\tau}\alpha)
    &= \sum_{\tilde{n}=0}^M \sum_{\tilde{m}=0}^M
    \frac{1}{\tilde{n}!}\frac{1}{\tilde{m}!}
    \left\langle
        \big(\sqrt{\kappa \tau} \sigma_\mathrm{chain}^+\big)^{\tilde{n}}
        \big(\sqrt{\kappa \tau} \sigma_\mathrm{chain}^-\big)^{\tilde{m}}
    \right\rangle
    e^{-\partial_x\partial_y}\Big|_{x=0=y} 
    (b^\dagger + x)^{\tilde{m}} |0\rangle\langle0| (b + y)^{\tilde{n}}\\
%
    &= \sum_{\tilde{n}=0}^M \sum_{\tilde{m}=0}^M
    \left\langle
        \big(\sqrt{\kappa \tau} \sigma_\mathrm{chain}^+\big)^{\tilde{n}}
        \big(\sqrt{\kappa \tau} \sigma_\mathrm{chain}^-\big)^{\tilde{m}}
    \right\rangle
    \sum_{k=0}^{\min(\tilde{n},\tilde{m})} (-1)^k
    \frac{%
        |\tilde{m}-k \rangle\langle \tilde{n}-k|
    }{%
        k!\sqrt{(\tilde{n}-k)!}\sqrt{(\tilde{m}-k)!}
    }.
\end{align}
Here, the right hand side is spanned by the truncated Fock space $\{|0\rangle,\dots,|M\rangle\}$, which is to say that $\rho_v$ generally is a $(M+1)$-state mixture of $M$-photon added coherent states in the short bin limit $\kappa \tau \ll 1$.

